Physical properties of more than one thousand brightest cluster galaxies detected in the Canada France Hawaii Telescope Legacy Survey

Brightest cluster galaxies (BCGs) are very massive elliptical galaxies found at the centers of clusters. Their study gives clues on the formation and evolution of the clusters in which they are embedded. We analysed here in a homogeneous way the properties of a sample of more than one thousand BCGs in the redshift range 0.15 < z < 0.7, based on images from the Canada France Hawaii Telescope Legacy Survey. Based on the cluster catalogue of 1371 clusters by Sarron et al. (2018), we applied our automatic BCG detection algorithm and identified successfully 70% of the BCGs in our sample. We analysed their 2D photometric properties with GALFIT. We also compared the position angles of the BCG major axes with those of the overall cluster to which they belong. We found no evolution of the BCG properties with redshift up to z = 0.7, in agreement with previous results by Chu et al. (2021), who analysed an order of magnitude smaller sample, but reaching a redshift z = 1.8. The Kormendy relation for BCGs is tight and consistent with that of normal elliptical galaxies and BCGs measured by other authors. The position angles of the BCGs and of the cluster to which they belong agree within 30 degrees for 55% of the objects with well defined position angles. The study of this very large sample of more than one thousand BCGs shows that they were mainly formed before z = 0.7, as we find no significant growth for the luminosities and sizes of central galaxies. We discuss the importance of the intracluster light in the interpretation of these results. We highlight the role of image depth in the modelisation of the luminosity profiles of BCGs, and give evidence for the presence of an inner structure which can only be resolved on deep surveys with limiting apparent magnitude at 80% completeness m80 > 26 mag/arcsec2.

==> tab_sersic.tex <==
\begin{table*}[htbp]
\setcounter{table}{1}
\begin{minipage}{1.\textwidth}
\begin{center}
  \caption{Parameters obtained from fitting the luminosity profiles with a single S\'ersic component. The columns are: full cluster name, image type (original image or ICL subtracted image), absolute magnitude, mean effective surface brightness, effective radius, S\'ersic index, elongation (ratio of the major to minor axis), position angle.}
  \label{tab:tab1}
\begin{tabular}{ c  c | c  c  c  c }   \hline
Name & Image type & m$_{\rm ABS}$ & $<\mu_{\rm e}>$ & R$_{\rm e}$ & n  \\ % table heading
 & & (mag) & (mag/arcsec$^{2}$) & (kpc) &   \\
\hline                                   % inserts single horizontal line
  \multirow{2}{*}{ABELL 2744}  & 	  Original  & -25.471  &   23.168  &      60.600 &    6.83   \\
   &    Original - ICL     & -24.461  &   20.745  &      12.471 &    2.97    \\
   \hline
  \multirow{2}{*}{ABELL 383}   &    Original  & -25.293  &   20.716  &      21.837 &    2.71    \\
   & 	  Original - ICL     & -25.043  &   20.257  &      15.752 &    2.11  \\
   \hline
  \multirow{2}{*}{MACS J0416.1-2403}   &    Original  & -25.274  &   22.173  &      30.626 &    3.97   \\
    &    Original - ICL     & -25.164  &   22.263  &      30.351 &    3.85  \\
\hline
  \multirow{2}{*}{ABELL 611}   &    Original  & -25.630  &   21.742  &      34.749 &    3.01   \\
   & 	  Original - ICL     & -25.240  &   21.106  &      21.671 &    2.06   \\
  \hline
  \multirow{2}{*}{MACS J1115.9+0129}   &    Original  & -26.422  &   25.412  &      247.310 &   7.15  \\
   & 	  Original - ICL     & -24.852  &   21.927  &      24.113 &    2.67   \\
   \hline
  \multirow{2}{*}{MACS J1149+2223}   &    Original  &          &           &             &        \\
   & 	  Original - ICL     & -25.347  &   22.874  &      35.737 &    2.41 \\
   \hline
  \multirow{2}{*}{RX J2129.6+0005}    &    Original  & -25.966  &   22.865  &      74.153 &    3.98   \\
 & 	  Original - ICL     & -25.316  &   21.648  &      31.384 &    2.29    \\
 \hline
  \multirow{2}{*}{MS 2137}     &    Original  & -25.128  &   20.572  &      15.487 &    2.58   \\
     &    Original - ICL     & -24.878  &   20.162  &      11.429 &    2.00    \\

\hline         %inserts single line
\end{tabular}
\end{center}
\end{minipage}
\end{table*}


